Beware the Normative Fallacy

Behavioral research can provide important insights for SE practices. But in performing it, many studies of SE are committing a normative fallacy - they misappropriate normative and prescriptive theories for descriptive purposes. The evidence from reviews of empirical studies of decision making in SE suggests that the normative fallacy may is common. This article draws on cognitive psychology and behavioral economics to explains this fallacy. Because data collection is framed by narrow and empirically invalid theories, flawed assumptions baked into those theories lead to misleading interpretations of observed behaviors and ultimately, to invalid conclusions and flawed recommendations. Researchers should be careful not to rely solely on engineering methods to explain what people do when they do engineering. Instead, insist that descriptive research be based on validated descriptive theories, listen carefully to skilled practitioners, and only rely on validated findings to prescribe what they should do.

==> TABLE.tex <==



\vspace{0.5cm}


\noindent \textbf{Ideal Map 1}\\
The map was created by the requirements engineer and one of the CSH experts. It contained the requirements engineer’s observations from her previous discussions with the HomeSound development team, third-sector organizations, and families and caretakers of elderly people. Among other things, the map identified the elderly as the main \textit{beneficiary} and stated the \textit{purpose} as to increase their independence, allowing them to stay home longer. It also set the elderly’s ‘independence and well-being levels’ and he ‘number of years at living alone at home’ as a \textit{measurement of improvement}. We also assumed that if their well-being increased, this would reduce the  ‘number of distressed calls from elderly people’ to their caretakers, and therefore this could be taken as a possible \textit{guarantor of success} Space constraints prevents us from discussing the maps in detail. 
Reflection revealed, among other things, that we needed to consult the notes of previous conversations with stakeholders to more accurately reflect  their needs needs. This first map was built from the \textbf{selective memory} of the requirement engineer and most likely represented the \textbf{privileged views} of those developing the system. We also felt the need to involve a third researcher on the critique of the maps, a third party that could help reconcile and synthesize the dialogue, in lieu of more thorough participant involvement.  

\vspace{0.5cm}
\noindent \textbf{Ideal Map 2}\\
The map was created after the consultation of the notes from previous meetings and interviews with stakeholders. The new map added the families as a \textit{primary beneficiary} and the society and the healthcare system as a \textit{ second}, extending the \textbf{boundaries} of the system. In the \textit{purpose}, it  included the peace of mind of families. It also reviewed the concept of well-being and independence, among other things.
Reflection  on the validity of our \textit{measurements of success} made us to realize that we needed to get input from professionals with expertise on elderly people. For Ulrich, relying on incomplete or dogmatic perspectives is a major ‘\textbf{source of deception}’, and can be a \textit{false guarantor }that harms our understanding of the situation, and our systems design \cite{ulrich1983critical}. It also raised a number of questions, such as: What are the boundaries of the system? Is ‘years at home’ a real measure of well-being? What about uninvolved family members? Should the purpose be to increase independence or self-determination? Do people really understand the implications of the technology? Why have we observed a blind trust in technology in our conversations with stakeholders? What if the elderly cannot be the decision maker? The latter is raises important issues of \textit{fair representation of the concerns of those at risk of marginalization}.

\vspace{0.5cm}
\noindent  \textbf{Ideal Map 3}\\
The map  integrated the views of a social worker and a psychologist, both specialized on the elderly. The interviews highlighted several issues, including that the system did not increase independence,  but security (as it cannot meet their physical and emotional needs) and that the number of calls from the elderly were not a \textbf{false guarantor of success}. We also learned about  common behaviors, coping mechanisms, the importance of a trusted person, and several scales for measuring well-being of elderly people and their caretakers. The new map included new \textit{ measures of success} (e.g. social support, anxiety of the caretaker, early signs of dementia) and professional scales normally used in psychology and social care to measure them, an extended list of\textit{ decision makers} and \textit{sources of knowledge}.
Reflection raised doubts regarding the measurement of self-determination and early signs of dementia, and brought up questions such as: Is RE missing critical reflection? What should the the role of  CSH in RE be? %% Did it? Those are odd questions. Of course it does...?


\vspace{0.5cm}
\noindent \textbf{Ideal Map 4}\\\
The map  was developed after an interview with an practical philosopher, specialised on the impact of technological projects in ethics and privacy. We discussed issues such as: How do you frame care and wellbeing? What is the amount of trust required from the user? Can over-reliance of families lead to less ‘human touch’ and potentially reducing wellbeing? Can the technology can reduce the autonomy of the elderly, who have the right to decide when to get help? Can third parties be interested in this data? The last two being interesting examples of \textbf{power and politics}. Finally, we learned about the importance of public debate on such technologies, and about techniques from practical philosophy for uncovering stakeholder ethics, morals and values.  The new map included  autonomy as a \textit{primary aim}, a better definition of self-determination, the general public as a \textit{desired expert}, institutions that are interested in data as a commodity as an \textit{undesired expert}, and possible \textit{worldviews} about being old, supporting the elderly, living the good life, and surveillance technology.
Reflection led us to realise we had been more concerned with people's perception than security, assuming this was something more easily solvable. Hence, we chose to interview a security expert.


\vspace{0.5cm}
\noindent \textbf{Ideal Map 5}\\
The map integrated the opinions of a IT security specialist who works with security audits of technological solutions.  He highlighted that sound monitoring may not be the best solution to the problem due to the intrinsic risks of having microphones in the house. We learned about the different privacy and security risks of these type of devices and were recommended a security audit when the system is under development. The new map included the \textit{desired skills} that a security expert could bring to the project, a new \textit{guarantor of success} ( the number of vulnerabilities discovered in recurrent security audits), and several risks and possible measures.    
Reflection led us to a discussion on the role of risk assessment in CSH and whether it could lead to an oversimplification of the problem and the risk of overlooking the important issue of  moral justification of the project. We also reflect on how the insights from CSH were different from our previous experiences with RE techniques, and on how we could integrate these insights into RE. This led us to decide to attempt to map the CSH findings to the Volere framework. 


\vspace{0.5cm}
\noindent  \textbf{Ideal Map 6}\\
The map incorporated the insights derived from attempting to translate the findings of the CSH to a Volere specification. These included classifying previous secondary aims as \textit{unrealistic aims} (as they were out of the scope of the technical system) and improving rationale, relationship and consistency for items across different sections of the ideal map. Reflection showed us that there seems to be value in iterating between standard RE and CSH. 

The CSH process still continues, now to integrate the views of elderly people. But at the time of writing no new version of the ideal had been generated from the later inputs.  



